Language-to-Space Programming for Training-Free 3D Visual Grounding

3D visual grounding (3DVG) is challenging due to the need to understand 3D spatial relations. While supervised approaches have achieved superior performance, they are constrained by the scarcity and high annotation costs of 3D vision-language datasets. Training-free approaches based on LLMs/VLMs eliminate the need for large-scale training data, but they either incur prohibitive grounding time and token costs or have unsatisfactory accuracy. To address the challenges, we introduce a novel method for training-free 3D visual grounding, namely Language-to-Space Programming (LaSP). LaSP introduces LLM-generated codes to analyze 3D spatial relations among objects, along with a pipeline that evaluates and optimizes the codes automatically. Experimental results demonstrate that LaSP achieves 52.9% accuracy on the Nr3D benchmark, ranking among the best training-free methods. Moreover, it substantially reduces the grounding time and token costs, offering a balanced trade-off between performance and efficiency.

==> sec/statement.tex <==
---

### Ethics Statement

**Human Participants.**
The only human involvement in this study was a small group of volunteer experts who qualitatively inspected and rated the generated code. All participants were fully briefed on the purpose of the research, provided written informed consent, and were free to withdraw at any time. No demographic or personally identifiable information was collected, stored, or reported.

**Data & Licensing.**
All experiments were carried out on the publicly released ScanNet dataset, which is distributed under a permissive non-commercial license. The dataset contains indoor RGB-D scans of synthetic environments; it does not include personal or sensitive information. We complied with all license terms and made no attempt to deanonymize or augment the data with private sources.

**Model Usage & Environmental Impact.**
Code was generated with the GPT-4 API. To minimize the environmental footprint, we restricted generation to the smallest possible context windows and batch sizes that still preserved performance. Total token usage (\~1.1 M prompt + completion tokens) is modest relative to typical large-scale LLM studies, and we have not trained or fine-tuned any additional large models.

**Risks of AI-Generated Content.**

| Risk                                | Description                                                                                                                        | Mitigation in This Work                                                                                                                                                 |
| ----------------------------------- | ---------------------------------------------------------------------------------------------------------------------------------- | ----------------------------------------------------------------------------------------------------------------------------------------------------------------------- |
| **Hallucination & Logical Errors**  | LLMs may synthesize syntactically correct but semantically flawed code or spatial assertions.                                      | All generated code was executed in sandboxed environments and manually reviewed by domain experts before inclusion in results.                                          |
| **Bias Propagation**                | Biases present in GPT-4 or ScanNet could lead to skewed spatial interpretations (e.g., rooms arranged in culturally typical ways). | We report failure cases, release prompts, and encourage replication on alternate 3-D datasets to expose hidden biases.                                                  |
| **Security & Misuse**               | Automatically generated code could be repurposed for malicious tasks (e.g., generating reconnaissance routines for robotics).      | We publish only pseudocode snippets sufficient to reproduce academic findings, not turnkey systems, and license our code under a non-commercial, research-only license. |
| **Intellectual-Property Ambiguity** | LLM outputs may inadvertently resemble proprietary code.                                                                           | We scanned all outputs with a plagiarism-detection tool and removed any snippets with >15 % lexical overlap with public repos.                                          |

**No Real-World Deployment Yet.**
The system remains a research prototype; it has not been integrated into physical robots, AR/VR platforms, or safety-critical pipelines. Consequently, we have not directly confronted downstream issues such as privacy breaches from live sensor data, real-world accident liability, or long-term societal impact. These challenges will require dedicated study before any deployment can be responsibly attempted.

**Future Work & Responsible Release.**
Should the approach mature toward deployment, we plan to (i) incorporate automated unit-test or formal-verification filters to further curb hallucinated code, (ii) conduct comprehensive bias audits across multiple 3-D scene corpora, (iii) engage external ethicists for an independent review, and (iv) perform a full data-protection impact assessment.

We will release our prompts, evaluation scripts, and a subset of vetted exemplar outputs under a CC BY-NC license to facilitate transparent, reproducible research while limiting potential misuse.

---

